A Survey on Deep Learning for Theorem Proving

Theorem proving is a fundamental aspect of mathematics, spanning from informal reasoning in natural language to rigorous derivations in formal systems. In recent years, the advancement of deep learning, especially the emergence of large language models, has sparked a notable surge of research exploring these techniques to enhance the process of theorem proving. This paper presents a comprehensive survey of deep learning for theorem proving by offering (i) a thorough review of existing approaches across various tasks such as autoformalization, premise selection, proofstep generation, and proof search; (ii) an extensive summary of curated datasets and strategies for synthetic data generation; (iii) a detailed analysis of evaluation metrics and the performance of state-of-the-art methods; and (iv) a critical discussion on the persistent challenges and the promising avenues for future exploration. Our survey aims to serve as a foundational reference for deep learning approaches in theorem proving, inspiring and catalyzing further research endeavors in this rapidly growing field. A curated list of papers is available at https://github.com/zhaoyu-li/DL4TP.

==> content/jack.tex <==

% Theorem proving is a key aspect of mathematics, encompassing a spectrum from informal reasoning in natural language to rigorous derivations in formal systems. The recent advancement of deep learning, especially the advent of large language models, has sparked a notable surge of research harnessing these techniques to enhance the process of theorem proving. Despite the burgeoning interest, this evolving field presents a complex and diverse landscape without a unified framework for evaluating the efficacy of existing approaches. In this paper, we provide the first comprehensive review of the current state of deep learning for theorem proving, systematically analyzing the variety of prediction tasks, methodologies, datasets, and evaluations in the literature. We also highlight the considerable advancements and enduring challenges within this field and propose potential avenues for further research. 


% Proving theorems is the central objective of mathematical reasoning. Computers can be employed to assist proof development in a number of manners, from automated theorem proving (ATP) to autoformalization.  The emergence of deep learning (DL) has opened new opportunities to leverage learning-based reasoning for theorem proving. A number of such proposals have been presented and implemented in recent years, and the field is developing extremely rapidly, especially following the development of large language models (LLMs). In this paper, we provide the first comprehensive review of deep learning for theorem proving. We analyze a variety of prediction tasks, methodologies, datasets, and evaluation schemes from the literature. We also propose potential avenues for further research. 

% Proposed change from Jack
% Theorem proving is a key aspect of mathematics, encompassing a spectrum from informal reasoning in mathematical language to rigorous derivations in formal systems. The recent advancement of deep learning, especially the advent of large language models, has sparked a notable surge of research harnessing these techniques to enhance the process of theorem proving. However, the lack of a unified framework for classifying and evaluating the approaches complicates identifying the true developments and obstacles in theorem proving. In this paper, we provide the first comprehensive survey of deep learning for theorem proving by offering i) a meticulous classification of theorem-proving tasks across diverse problem types, languages, and difficulty spectrums; ii) an in-depth dissection of deep-learning-based theorem-proving approaches including autoformalization, premise selection, proof generation, and proof search, and proof data synthesis; iii) a detailed evaluation and comparison of these methodologies against their performance on the datasets; iv) a summary of significant advancements and enduring obstacles within this field and potential avenues for future endeavors in this field.
% Through this work, we aim to establish a cornerstone for deep learning with theorem proving and provide a structured foundation to inspire future endeavors in this field.



% Autoformalization aims to convert theorem statements and proofs from natural language into machine-checkable formalizations, requiring a profound understanding of both informal and formal mathematics to bridge the logical gap inherent in natural language's ambiguity. This process enhances formal theorem-proving by providing automated theorem provers with informal proof sketches \citep{jiang2022draft}. While initial approaches utilized probabilistic semantic parsing \citep{kaliszyk2015learning} and type-checking/ATP for translating informal LaTeX text into Mizar language \citep{kaliszyk2017automating}, the field evolved with the utilization of sequence-to-sequence (Seq2Seq) models \citep{cunningham10towards} like Recurrent Neural Networks (RNN) and Long Short Term Memory (LSTM) networks, facing challenges in managing long-term dependencies due to their sequential nature. The introduction of attention-based models, especially transformers, marked a significant advancement, allowing for effective parsing and comprehension of formal languages. This progress enabled the use of large language models (LLMs) such as Codex and PaLM \citep{wu2022autoformalization} for autoformalization, demonstrating their capability to translate a considerable portion of mathematical competition problems into formal specifications in Isabelle/HOL accurately (25.3\%) and enhancing neural theorem proving performance. LLEMMA \citep{azerbayev2023llemma}, further pretrained on Proof-Pile-2, exemplifies the potential of LLMs in mathematics by outperforming known models in formal theorem proving. The effective training of neural translation methods for autoformalization relies heavily on a substantial volume of aligned informal and formal mathematical datasets. Unfortunately, the limited availability of formal mathematical data poses a significant challenge, with \textit{the Archive of Formal Proofs} representing the largest formal corpus at a mere 328MB. Inspired backtranslation \citep{sennrich-etal-2016-improving}, a groundbreaking approach to mitigate this data scarcity issue is presented through distilled backtranslation (informalization) \citep{azerbayev2024proofnet}, which translates formal statements back to natural language, creating synthetic training pairs and eliminating the dependency on parallel datasets. Furthermore, techniques like few-shot prompting, chain-of-thought (CoT) prompting \citep{wei2022chain}, and self-consistency \citep{wang2022self} show promise in generalizing from limited input samples to novel queries. However, the susceptibility of few-shot learning to overfitting due to its dependency on specific input examples is addressed by prompt-retrieval methods \citep{azerbayev2024proofnet}, employing nearest-neighbor searches to identify the most relevant mathlib examples for more accurate model training. Additionally, postprocessing methods, including the vacuous statement filter and self-critique filter \citep{zhou2023don}, enhance the reliability of translated statements by eliminating unfaithful ones through ATP checks for vacuous clauses and language model evaluations for statement fidelity. These advancements collectively signify a leap forward in the autoformalization field, laying the groundwork for more efficient and accurate translation of mathematical texts into formal languages.





% Jack Sun:
% Draft: 
% Category: Autoformalizing theorem statement / proof
% Semantic Parsing (variable, definition mapping)
% Describe the existing seq2seq model (rnn, lstm), attention-based model (PaLM, Codex, GPT)
% Pretraining and Finetuning the models on the aligned data ()
% Prompt tricks (few-shot, CoT, Self-consistency)
% Lack of aligned data: Distilled backtranslation/informalizatiion (to generate more data).
% Postprocessing: Filter out the syntactically incorrect/vacuous statement by proof assistant, or ask LLM to identify the incorrect translation using 


% The largest formal math corpus is only 180 MB (Archive of Formal Proofs).
% MULTILINGUAL MATHEMATICAL AUTOFORMALIZATION: use back-translation to avoid curating large dataset

% Although LLMs are capable of writing informal proofs for complicated mathematical theorems, they may make imperceptible logical errors or loopholes due to the inherent ambiguity of natural language. 
% Autoformalization aims to automatically translate mathematics in natural language into machine-checkable theorem statements and proofs, which bridges the informal and formal theorem proving and guarantees 100\& correctness of proofs. We provide a contrastive example of informal and formal theorem statement and proof of the Polar Decomposition Theorem from ProofNet \citep{azerbayev2024proofnet} as below:

% Autoformalization with LLM is a challenging task due to the scarcity of aligned data between formal and informal mathematics. Thanks to its capability of capturing and generalizing the patterns in the prompt, we can utilize few-shot learning in autoformalization. That is, we prompt the LLM by the instruction message along several pairs of informal and formal propositions/proof for training and query the formalization of target propositions/proof. [TODO: Add more methods] \\
% It is important to ensure the informal and formalized theorem statements are indeed semantically equivalent, which is nontrivial as it requires a ground truth formalized theorem for the informal one. Before this, we can pre-check the formalized statement [TODO: Self-contradictory-check]



\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{1in}p{0.7in}llp{0.7in}l}
\toprule[1pt]
Type & Name & Language & Domain & Size & Note \\
\midrule
TPTP & SMT & University & & Formal&\\
miniF2F& Isabelle  &  High School Olympiad & 488 & Formal & \\ 
LISA & Isabelle  &  High School Olympiad & 183K & Formal & \\ 
IsarStep & Isabelle & University & 830K & Formal & \\ 
LeanDojo & Lean  &  University & 100K & Formal  & \\ 
FIMO & Lean  &  High School Olympiad & 149 & Formal & \\ 
ProofNet & Lean & University & 371 & Formal \& Informal & \\
Holist & \\
HolStep & HOL Light & [TODO: Find it!] & 2.2M & Formal& \\
% MATH & Natural Language & High School Olympiad & 12.5K & Informal& \\
CoqGym & Coq & Software \& Hardware Projects& 71K& Formal& \\
GamePad& Coq & Feit-Thompson Dataset& 1.6K& Formal & \\
MLFMF & Lean\&Agda& & 250K& Informal \& Formal& \\
INT & Lean & Inequalities& & Formal& \\
FormalGeo & \\
DeepMath & \\
NaturalProofs \\
HOList & \\
mathlib \\
Metamath library
PRISM \\
% proof-pile \\
% proof-pile-2 \\
TRIGO \\
\bottomrule[1pt]
\end{tabular}
}
\caption{Datasets for Theorem Proving}
\label{tab:datasets}
\end{table}




%For instance, \citet{mma} uses GPT-4 to informalize all the mathematical statements in Archive of Formal Proofs~\footnote{https://www.isa-afp.org/} of Isabelle and \texttt{mathlib}~\citep{mathlib} of Lean.

\subsection{Data Collection}
\label{sec:data_collection}
\textbf{Libraries and Frameworks} 
Growing community efforts to build formal mathematical libraries lays the foundation of learning-based theorem proving. The TPTP dataset~\citep{tptp} is the first comprehensive mathematical library capable of evaluating all first-order automated theorem provers. With the rise of ITPs in theorem proving, more projects are established, such as Metamath~\citep{megill2007metamath}, Mizar Mathematical Library~\citep{mizar}, Flyspeck ~\citep{hales2006introduction}, Isabelle Archive of Formal Proofs~\citep{DiskPaxos-AFP}, Coq standard library~\citep{coq}, HOL Light library~\citep{hol_light}, and Lean Mathlib~\citep{mathlib}.\\
\textbf{(Informal-Formal Datasets)} Handcrafted datasets are the ones manually formalized from existing informal mathematical data. miniF2F~\citep{zheng2021minif2f} is the first cross-system handcrafted dataset of 488 theorems from high-school competition for evaluation. ProofNet~\citep{proofnet} and FIMO~\citep{fimo} are follow-up manually-built Lean 3 datasets for undergraduate mathematics and challenging IMO problems, respectively, but these three datasets do not include formal proofs. The IPC dataset ~\citep{bordg2022parallel} is the Isabelle dataset of 500 informal and formal statements and proofs. Manually curating parallel datasets is extremely challenging due to extensive labor, until ~\citet{mma} proposed to informalize the formal mathematics via LLMs and created the large multi-domain dataset MMA from the Isabelle Archive of Formal Proofs and Mathlib.
\textbf{Formal-only Datasets} With the broad spectrum of raw formal data from ITP libraries and software projects, numerous formal datasets are created for machine-learning theorem-proving environment. Datasets like HolStep~\citep{holstep}, IsarStep~\citep{li2020isarstep}, LeanStep~\citep{pact}, LeanDojo~\citep{leandojo} focus on stepwise premise-selection and tactic-prediction for data extraction, while gym-like datasets such as CoqGym~\citep{yang2019learning}, PISA~\citep{lisa}, LeanGym~\citep{curriculum_learning} focus on whole proofs by interacting with proof assistant. ~\citet{traditional_ps_2} applied traditional ML methods like corpus analysis and kernel method for minimal dependency analysis, and MagnusHammer~\citep{magnushammer} uses transformer to select premises, but these datasets only have (proof state, relevant premise) pairs. MLFMF~\citep{mlfmf} represents a proof by directed acyclic graph. UniGeo~\citep{unigeo} and FormalGeo~\citep{zhang2023formalgeo} only include geometry problems. 
\textbf{Informal-only Datasets}
\\The recent advancements in LLM urge the need for natural language mathematical datasets. 
~\citet{ferreira2020natural} proposed the concept of natural premise selection and constructed NL-PS from ProofWiki to support the training and evaluation of informal theorem proving, followed by NaturalProofs~\citep{naturalproofs} and MATcH~\citep{li2023bert} datasets of informal statement-proof pairs that encompasse a broader and deeper coverage of mathematical sources. To improve reasoning abilities of large language models, High-quality and large-scale corpora of billions of tokens were introduced via meticulous data collection from CommonCrawl webpages, including the 8B Proof-Pile~\citep{proofnet}, 9.5B MathPile~\citep{wang2023generative}, 14.7B OpenWebMath~\citep{paster2023openwebmath}, 55B Proof-Pile-2~\citep{llemma} and 120B DeepSeekMath~\citep{deepseekmath}. 


% Datasets are fundamental in the development and evaluation of ML-based theorem provers, with sources like arXiv, ProofWiki, and StackExchange offering a wealth of informal mathematical data across numerous disciplines. This diverse array of datasets, spanning languages such as Natural Language, Mizar, HOL, Isabelle, and Lean, is derived from a mix of informal and formal mathematical corpora. These datasets are generally categorized into two main types: (i) those manually curated or extracted from large-scale mathematics and software verification projects, aimed at training or evaluating theorem provers, and (ii) synthetic datasets created through algorithmic processes to support theorem proving tasks. Such datasets underpin the training of models to navigate the complex landscape of mathematical information retrieval, theorem statement matching, and proof generation, highlighting the challenges and potential of ML in automated theorem proving.

f 4.4M premise selection instances







% existing sources such as arXiv, StackExchange and text books offer a plethora of raw mathematical data. There is also a line of work that leverages large corpora with billions of tokens with informal and formal math data, and code for pre-training. These includes WebMath~\citep{pact} 35B tokens,  Proof-Pile~\citep{proofnet} (8.3 B tokens) mainly from arXiv.math and Stack Exchanges, MathPile (9.5B) OpenWebMath 14.7B tokens, Proof-Pile-2~\citep{llemma} (55B, code, proofpile ArXiv (Computer, 2023)) and DeepSeekMath (120 B tokens). internlm 125b.

% Beyond specific datasets, there is a wealth of raw mathematical data available from sources such as arXiv, StackExchange, and textbooks. A new line of research has emerged, leveraging massive corpora containing billions of tokens encompassing both informal and formal mathematical data. This includes WebMath with 35 billion tokens, Proof-Pile (8.3 billion tokens) primarily from arXiv.math and Stack Exchange, MathPile (9.5 billion tokens), OpenWebMath (14.7 billion tokens), Proof-Pile-2 (55 billion tokens), and DeepSeekMath (120 billion tokens), among others. These resources are instrumental for pre-training models in the field of automated theorem proving, offering unprecedented scale and diversity.


% with the help of GPT-4. ProofNet formalize the statements

% This includes miniF2F 448, Fimo and ProofNet 371, IPC 500 isabelle proofs to match nl statement. 
% there is a wide range of formal libraries and verification projects, providing a good source. The existing



% On the other hand, human experts have manually formalized a range of mathematical theorems or verification projects, accumulating a wide variety of formal libraries. These includes TPTP, the coq standard library, Archive of Formal Proofs~\citep{DiskPaxos-AFP}, and Lean Mathlib~\citep{mathlib}. All of these provides a range of instances can be serves datasets for theorem proving or can be manually formalized as datasets. 
% A line of work extracted and cleaned formal theorems and proofs from them. GamePad uses the data from Feit-Thompson theorem, contains 83k proof steps (1602 lemmas). CoqGym 71K
% human-written proofs from 123. PRISM build dataset for proof repair. IsarStep contains 830k training examples from afp. pisa 183k theorems, 4k testing, Isabelle standard library [11] and the Archive of Formal Proofs (AFP). maghushumer 4.4M premise selection instances,  For Lean, LeanStep extract theorems from mathlib, lean dojo, 8,734 theorems/proofs extracted from mathlib. holstep from ts multivariate analysis library (Harrison, 2013), as well as the formal proof of the Kepler conjecture. gpt-f metamath




% Aligned datasets consist of parallel informal and formal mathematics, such as the manually-curated miniF2F~\citep{zheng2021minif2f} dataset, which offers 488 high-school \lm{also university/IMO/etc} competition theorems for cross-system evaluation. Lean 3 datasets like ProofNet~\citep{proofnet} and FIMO~\citep{fimo} extended this to undergraduate and IMO problems, though without formal proofs. The IPC dataset~\citep{bordg2022parallel} made a notable advance by including 500 paired informal and formal proofs. 




% IPC~\citep{ipc} aims to provide aligned Natural Language and Isabelle proofs. 

% The plethora of data from ITP libraries has led to diverse datasets aimed at ML-driven theorem proving. Early efforts included the MPTP2078 dataset~\citep{alama2014premise} for premise selection, followed by collections focusing on tactic prediction and interactive proof construction like HolStep~\citep{holstep} and lean-gym~\citep{curriculum_learning}. Domain-specific datasets, such as UniGeo~\citep{unigeo}, address geometry problems ranging from textbook level to IMO challenges.



% The evolution of formal mathematical libraries has significantly advanced learning-based theorem proving. Datasets like TPTP~\cite{tptp} have been critical for evaluating first-order automated theorem provers, further enhanced by Interactive Theorem Provers (ITPs) libraries and projects such as Metamath~\citep{megill2007metamath}, Archive of Formal Proofs~\citep{DiskPaxos-AFP}, and Lean Mathlib~\citep{mathlib}.



% The rise of large language models (LLMs) has highlighted the importance of natural language mathematical datasets for informal theorem proving. Initiatives like NL-PS from ProofWiki~\citep{ferreira2020natural} and subsequent datasets including NaturalProofs~\citep{naturalproofs} offer informal statement-proof pairs across various mathematical areas. Additionally, large-scale corpora such as the 8B Proof-Pile~\citep{proofnet} and 120B DeepSeekMath~\citep{deepseekmath} have been assembled from web sources to enhance LLM reasoning capabilities.

% The evolution of formal mathematical libraries has been instrumental in learning-based theorem proving. Initiatives in formal mathematical like the TPTP dataset~\cite{tptp} have paved the way by offering comprehensive resources to evaluate first-order automated theorem provers. This has been further enriched by the advent of Interactive Theorem Provers (ITPs), leading to the establishment of foundational projects such as Metamath~\citep{megill2007metamath}, the Mizar Mathematical Library~\citep{mizar}, Flyspeck~\citep{hales2006introduction}, the Isabelle Archive of Formal Proofs~\citep{DiskPaxos-AFP}, the Coq standard library~\citep{coq}, the HOL Light library~\citep{hol_light}, and Lean Mathlib~\citep{mathlib}.

% Creating handcrafted datasets involves meticulous translation of informal mathematical content into formalized data. Notably, miniF2F~\citep{zheng2021minif2f} emerged as the inaugural dataset providing 488 theorems from high-school competitions for cross-system evaluation. This was followed by the development of Lean 3 datasets such as ProofNet~\citep{proofnet} and FIMO~\citep{fimo}, targeting undergraduate mathematics and International Mathematical Olympiad (IMO) problems, respectively. However, these three lacked formal proofs. The IPC dataset~\citep{bordg2022parallel} represents a significant stride with its collection of 500 paired informal and formal statements and proofs. The labor-intensive nature of manually curating such parallel datasets saw innovation with the introduction of the MMA dataset by ~\citet{mma}, utilizing LLMs to bridge formal and informal mathematics from the Isabelle Archive of Formal Proofs and Mathlib.

% The abundant formal data from ITP libraries and software projects facilitated the creation of diverse datasets tailored for ML-driven theorem proving. In the early stage, ~\citet{alama2014premise} created the MPTP2078 dataset for premise-selection tasks by traditional corpus analysis. Then, collections such as HolStep~\citep{holstep}, IsarStep~\citep{li2020isarstep}, LeanStep~\citep{pact}, and LeanDojo~\citep{leandojo} concentrate on the premise selection and tactic prediction tasks, while interactive platforms like CoqGym~\citep{yang2019learning}, PISA~\citep{lisa}, and LeanGym~\citep{curriculum_learning} focus on engaging with proof assistants for full-proof construction. Other datasets like Magnushammer~\citep{magnushammer} used transformers to generate (proof state, relevant premise) pairs, and the MLFMF~\citep{mlfmf} stores data in directed multi-graph. Domain-specific datasets in geometry include UniGeo~\citep{unigeo} and FormalGeo~\citep{zhang2023formalgeo} with difficulty ranging from high-school textbooks to IMO-level problems.

% The surge in large language model (LLM) advancements has underscored the need for comprehensive natural language mathematical datasets. Initiatives ~\citet{ferreira2020natural} proposed the concept of natural premise selection and constructed NL-PS from ProofWiki to support the training and evaluation of informal theorem proving, followed by NaturalProofs~\citep{naturalproofs}, and MATcH~\citep{li2023bert} datasets featuring informal statement-proof pairs, spanning a wide and in-depth array of mathematical topics. Additionally, the quest for enhancing LLM reasoning capabilities has led to the assembly of large-scale corpora, including the 8B Proof-Pile~\citep{proofnet}, 9.5B MathPile~\citep{wang2023generative}, 14.7B OpenWebMath~\citep{paster2023openwebmath}, 55B Proof-Pile-2~\citep{llemma}, and 120B DeepSeekMath~\citep{deepseekmath}, meticulously compiled from CommonCrawl webpages.






% Formal Part
% data extraction 

% manually formalized datasets (NL is given)

% large-scale proof datasets

% \\Early Attempt: MPTP2078~\citep{alama2014premise}: Premise Selection (Corpus Analysis and Kernel Methods) + ATP in Mizar.
% \\High School Olympiad Benchmark with informal+formal: miniF2F~\citep{zheng2021minif2f} (Metamath, Lean, Isabelle and HOL Light), FIMO~\citep{liu2023fimo} (Lean)
% \\Undergraduate Level with informal+formal: ProofNet (Lean)
% \\Data Extraction+ PS: LeanDojo~\citep{yang2024leandojo}
% \\Use autoformalization to create formal dataset: MLFMF~\citep{bauer2023mlfmf}, MMA~\citep{mma} (Informalization by By GPT4), 
% \\For Geometry Problem Solving: UniGeo~\citep{chen2022unigeo}, FormalGeo~\citep{zhang2023formalgeo}


% LeanDojo: Tools for data extraction and interacting with proof
% assistants have been crucial drivers of learning-based theorem proving. Existing tools and datasets
% can be divided by proof assistants: Coq has GamePad [51], CoqGym [9], and PRISM [52]; Isabelle
% has IsarStep [53] and PISA [15]; HOL Light has HOList [54] and HoLStep [55], and Lean has
% LeanStep [16] and lean-gym [19]. miniF2F [28] is the only cross-system dataset, with 488 theorems
% for evaluation. However, it does not have training theorems and is restricted to the domain of math
% olympiads.






% However, given the diverse setting of approaches, some work constrains the time budget of a prover while others may limit the attempt numbers.

% In evaluating proof step generation and search, methods often merge these aspects to measure a theorem prover's effectiveness through its success rate in proving theorems within a test set. However, the variety in experimental setups complicates direct comparisons. Some studies impose a time budget on the prover, while others restrict the number of proof attempts, highlighting the need for standardized or adaptable evaluation metrics to account for these differences.


% For proof step generation and proof search, current approaches often merge these processes to evaluate a theorem prover's effectiveness, typically measured by the success rate of theorems proved in a test set. However, this evaluation is complicated by the variety of methodologies employed; some limit the prover's time budget, while others restrict the number of proof attempts.


% but it is hard to accurately measure its performance.

% the performance of premise selection.

% The performance of premise selection is usually measured using metrics such as R@k (recall for the top k retrieved premises) and MRR (mean reciprocal rank), indicating the proportion and rank of human-used premises in a proof. This approach can introduce bias, as it may penalize valid selections applicable in alternative proofs, thus potentially misrepresenting the effectiveness of the selection process. Some approaches evaluate premise selection by combining it with proof generation to see its increased performance.

% pass @ k metric, which reflects the proportion of theorems proven successfully within k attempts. This metric also allows assessing proof autoformalization and premise selection techniques in theorem proving. For simplicity, we focus on the highest success rate achieved in each method, disregarding the number of proof attempts and computational budgets.

% The performance of autoformalization is primarily evaluated through manual equivalence checking, but it requires the expertise of both informal and formal backgrounds and is labor-intensive. Alternative metrics include the compilation rate and the BLEU score~\citep{bleu}. However, these proxy metrics may not accurately reflect logical accuracy: the former one overlook the compile-correct but semantic-wrong formalizations and the a latter one neglect the semantic-correct but different with the ground truth ones.


% In the realm of premise selection, the standard metric for evaluation is Recall @ k, which quantifies the accuracy of identifying relevant premises within the top-k selections, benchmarked against a predefined 'ground truth' proof. This methodology, however, introduces potential bias. Specifically, it may unjustly penalize valid premise selections that are pertinent to alternate proof strategies, thereby skewing the perceived efficacy of the selection mechanism.

% Regarding the generation of proof steps and the broader proof search process, the prevailing approach integrates these components to evaluate a theorem prover's overall performance. This is typically quantified by the success rate of theorem proofs within a given test set. It is important to note, though, that due to the varied methodologies employed, some studies impose restrictions on the prover's time budget, whereas others may limit the number of proof attempts. This variance highlights the necessity for a nuanced understanding of performance metrics in the context of autoformalization.






% \begin{wraptable}{r}{0.48\textwidth}
%   \centering
%   \vspace{-10pt}
%   \resizebox{0.48\textwidth}{!}{
%   \begin{tabular}{lcc}
%     \toprule[1pt]
%     {\bf Task/Dataset} & {\bf Accuracy} & {\bf Method} \\
%     \midrule\midrule
%     \textit{1. Autoformalization} & & \\
%     \midrule
%     ProofNet & 16.1\% & ~\citet{proofnet} \\
%     MATH & 25.3\% & ~\citet{autoformalization_llm}\\
%     \midrule\midrule
%     \textit{2. Premise Selection} & & \\
%     \midrule
%     LeanDojo & 38.4\% & ~\citet{leandojo}\\
%     % DeepMath & 31.0\% & ~\citet{ps_gnn_6}\\
%     NaturalProofs & 36.9\% & ~\citet{ps_contrastive}\\
%     \midrule\midrule
%     \textit{3. Proof Generation} & & \\
%     \midrule
%     miniF2F & 50.0\% & ~\citet{lego}\\
%     PISA & 71.0\% & ~\citet{magnushammer}\\
%     Mathlib & 77.1\% & ~\citet{curriculum_learning}\\
%     CoqGym& 17.2\% & ~\citet{passport}\\
%     TPTP & 84.6\% & ~\citet{ensemble}\\ 
%     Metamath set.mm &  58.8\% & ~\citet{htps}\\
%     \bottomrule[1pt]
%     \label{tab:performance}
%   \end{tabular}
%   }
%   \vspace{-10pt}
%   \caption{State-of-the-art methods by Task and Dataset. }
% \end{wraptable}
  %   \centering
  % \vspace{10pt}
  % \resizebox{0.48\textwidth}{!}{
  % \begin{tabular}{lc}
  %   \toprule[1pt]
  %   {\bf Method} & {\bf Success Rate (\%)} \\
  %   \midrule
  %   LEGO-Prover~\citep{lego}& 50.0\\ % pass @ 100
  %   HTPS~\citep{htps}& 41.0\\% pass@64, 232 A100 days (1 day training), 7 days solving 
  %   DSP~\citep{dsp}& 39.3\\ % 100 formalization attempts, timeout 120s (sledgehammer)
  %   lean-gym~\citep{curriculum_learning}& 36.6\\ % pass@8. One proof search requires 0.1 A100 Hour
  %   Magnushammer~\citep{magnushammer}& 34.0\\ % ~ 800 s for each problem
  %   Copra~\citep{copra}& 30.7\\ % pass @ 1 * 100 queries * 1200 timeout for each problem
  %   DS-Prover~\citep{dsprover}& 29.6\\ % pass @ 1. 10-minute timeout. evaluation took 7 days with 4 A100 GPUs
  %   ReProver~\citep{leandojo}& 26.5\\ % pass @ 1, 10-minute timeout on single problem. miniF2F evaluation took 2 days on 8 V100 GPUs.
  %   \bottomrule[1pt]
  % \label{tab:minif2f_performance}
  % \end{tabular}
  % }
  % \vspace{-10pt}
  % \caption{Theorem provers on miniF2F-test dataset.}
  % 
  % \vspace{-10pt}


  % In contrast, Thor with traditional premise selection methods in Sledgehammer~\citep{sledgehammer} only 

% improves previous Sledgehammer~\citep{sledgehammer} to proves more theorems

% proves 71\% theorems in PISA and 36.9\% and 37.3\% on miniF2F-valid and miniF2F-test, while using the traditional premise selection components in ATP~\citep{sledgehammer} can only prove 57\% theorems in PISA, and 28.3\% and 36.9\% on miniF2F-valid and miniF2F-test.


% Finely-tuned models based on BERT architecture have markedly outstripped conventional approaches in the domain of premise selection, showcasing enhanced performance and the capability to generalize across previously unseen data. For instance, the ReProver model, as outlined in Yang et al. (2023), exhibits a recall of 27.6% at 10 retrieved items (R@10) and a Mean Reciprocal Rank (MRR) of 0.24, significantly surpassing the BM25 algorithm's performance, which stands at 15.5% for R@10 and 0.14 for MRR in the context of retrieving unseen premises within the LeanDojo benchmark. Furthermore, when integrated with the Thor proofstep prediction model, the Magnushammer system demonstrates a remarkable capacity for theorem proving, achieving a success rate of 71% in the PISA dataset and 36.9% and 37.3% in the miniF2F-valid and miniF2F-test datasets, respectively. This performance is notably superior to that achieved using traditional premise selection mechanisms in Automated Theorem Provers (ATP), which have managed a theorem proving success rate of only 57% in PISA and 28.3% and 36.9% in the miniF2F-valid and miniF2F-test datasets, respectively. These advancements highlight the transformative potential of BERT-based retrieval models in enhancing the efficiency and accuracy of premise selection and theorem proving processes.


% Fine-tuned BERT-based retrieval models represent a significant leap over conventional methods in premise selection, demonstrating remarkable ability to generalize to unseen data. The contrast is stark when examining the performance of ReProver, which, through its adaptation of BERT, attains a Recall at k of 27.6% and a Mean Reciprocal Rank (MRR) of 0.24 on the LeanDojo benchmark for retrieving premises not encountered during training. This is a marked improvement over the BM25 algorithm, which secures a 15.5% R@10 and 0.14 MRR under the same conditions. The integration of these advanced retrieval models with proof step prediction systems, such as Thor, further underscores their efficacy. Magnushammer, leveraging this combination, successfully proves 71% of theorems in the PISA dataset and achieves accuracies of 36.9% and 37.3% on the miniF2F-valid and miniF2F-test sets, respectively. In contrast, systems employing traditional premise selection methods, akin to those found in ATP tools like Sledgehammer, exhibit lower success rates: 57% in PISA and 28.3% and 36.9% on miniF2F-valid and miniF2F-test sets, respectively. This comparison highlights not only the superior performance of fine-tuned BERT models in identifying relevant premises but also their potential to significantly enhance theorem proving processes when coupled with predictive modeling techniques.



% Vision
@String(CVPR= {Conference on Computer Vision and Pattern Recognition (CVPR)})
@String(ICCV= {International Conference on Computer Vision (ICCV)})
@String(ECCV= {European Conference on Computer Vision (ECCV)})
@String(IJCV = {International Journal of Computer Vision (IJCV)})
@String(BMVC= {The British Machine Vision Conference (BMVC)})
@String(TIP  = {IEEE Transactions on Image Processing (TIP)})
@String(WACV = {Winter Conference on Applications of Computer Vision (WACV)})

% AI/ML
@String(ICML = {International Conference on Machine Learning (ICML)})
@String(NIPS= {Neural Information Processing Systems (NeurIPS)})s
@String(ICLR = {International Conference on Learning Representations (ICLR)})
@String(IJCAI = {International Joint Conference on Artificial Intelligence (IJCAI)})
@String(AAAI = {AAAI Conference on Artificial Intelligence})
@String(KDD = {International Conference on Knowledge Discovery and Data Mining (KDD)})
@String(AISTATS = {International Conference on Artificial Intelligence and Statistics (AISTATS)})
@String(JMLR = {Journal of Machine Learning Research (JMLR)})
@String(PAMI = {IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)})

% Robotics
@String(ICRA = {International Conference on Robotics and Automation (ICRA)})

% NLP
@String(TACL = {Transactions of the Association for Computational Linguistics (TACL)})
@String(EMNLP = {Conference on Empirical Methods in Natural Language Processing (EMNLP)})
@String(EMNLP\_Findings = {Findings of the Association for Computational Linguistics: EMNLP})
@String(ACL = {Annual Meeting of the Association for Computational Linguistics (ACL)})
@String(ACL\_Findings = {Findings of the Association for Computational Linguistics: ACL})
@string{EACL = {European Chapter of the Association for Computational Linguistics (EACL)}}
@String(CL = {Computational Linguistics})
@String(NAACL = {Annual Conference of the North American Chapter of the Association for Computational Linguistics (NAACL)})
@String(NAACL\_Findings = {Findings of the North American Chapter of the Association for Computational Linguistics: NAACL})
@String(IJCNLP = {International Joint Conference on Natural Language Processing (IJCNLP)})
@String(SIGIR = {International ACM SIGIR Conference on Research and Development in Information Retrieval (SIGIR)})

% PL
@String(POPL = {Symposium on Principles of Programming Languages (POPL)})
@String(CAV = {International Conference on Computer Aided Verification (CAV)})
@String(TACAS = {International Conference on Tools and Algorithms for the Construction and Analysis of Systems (TACAS)})
@String(LPAR = {International Conference on Logic for Programming Artificial Intelligence and Reasoning (LPAR)})
@String(FMCAD = {International Conference on Formal Methods in Computer-Aided Design (FMCAD)})
@String(CADE = {International Conference on Automated Deduction (CADE)})
@String(AITP = {Conference on Artificial Intelligence and Theorem Proving (AITP)})

% Security
@String(CCS = {Conference on Computer and Communications Security (CCS)})
@String(SP = {Symposium on Security and Privacy})
@String(USENIXSecurity = {USENIX Security Symposium})

% Cognitive Science
@String(CogSci = {Annual Meeting of the Cognitive Science Society (CogSci)})

% Theory
@String(STOC = {Symposium on Theory of Computing (STOC)})

% HCI
@String(CHI = {Conference on Human Factors in Computing Systems (CHI)})

% Others
@String(FAT = {Conference on Fairness, Accountability, and Transparency (FAccT)})

@article{yamabe,
  title={The Yamabe Problem},
  author={Lee, John M and Parker, Thomas H},
  journal={Bulletin of the American Mathematical Society},
  year={1987}
}

@book{kakutani,
  title={Mathematical Apocrypha: Stories and Anecdotes of Mathematicians and the Mathematical},
  author={Krantz, Steven G},
  year={2002},
}

@article{tao,
  title={A Maclaurin Type Inequality},
  author={Tao, Terence},
  journal={arXiv preprint arXiv:2310.05328},
  year={2023}
}





% \begin{table}[h]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \midrule
% Prover/Dataset & Mathlib (train/test) & miniF2F (train/test) & ProofNet & PISA & Metamath & HOList & LeanDojo & MPTP2078\\\midrule
% lean-gym~\citep{curriculum_learning} & 75.8/77.1 & & & & & & & \\\midrule
% LEGO-Prover~\citep{lego} & & 57.0/50.0& & & & & & \\\midrule
% DS-Prover~\citep{dsprover} & -/58.8 & -/29.8 & 14.2 & & & & & \\\midrule
% Lyra~\citep{lyra} & & 55.3/51.2 & & & & & & \\\midrule
% DSP~\citep{dsp} & & 43.9/39.3& & & & & & \\\midrule
% MagnusHammer~\citep{magnushammer} & & 36.9/37.3 & & 71.0 & & & & \\\midrule
% HyperTree~\citep{htps} & & 58.6/41.0 & & & 68.6/58.8 & & & \\\midrule
% GNN~\citep{graph_representation} & & & & & & 49.95 & & \\\midrule
% Temperature Scaling~\citep{temperature} & & & & & & & 57.7& \\\midrule
% NIAGARA~\citep{ensemble} & & & & & & & & 73.0\\\midrule
% \end{tabular}}
% \caption{Proof Success Rate (\%) of various Theorem Provers on Datasets}
% \label{your-table-label}
% \end{table}






% \section{Appendix}
% You may include other additional sections here.




% \begin{table}[h]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|}
% \midrule
% Dataset & SOTA accuracy (valid/test) & Prover\\ \midrule
% Mathlib & 75.8/77.1 & lean-gym~\citep{curriculum_learning}\\ \midrule
% Minif2f & 57.0/50.0 & LEGO-Prover~\citep{lego} \\ \midrule
% ProofNet & 14.2 & DS-Prover~\citep{dsprover}\\ \midrule
% % on miniF2F test: 29.8, on MathLib 58.8

% % Lyra on miniF2F: 55.3/51.2
% % DSP on miniF2F: 43.9/39.3
% PISA & 71.0 & Magnushammer~\citep{magnushammer} \\ \midrule
% % Magnus+Thor on PISA: 71, on miniF2F: 36.9/37.3
% Metamath & 68.6/58.8 & HyperTree~\citep{htps} \\ \midrule
% % Metamath 68.6/57.4
% % miniF2F 58.6/41.0
% HOList & 49.95 & GNN~\citep{graph_representation} \\ \midrule
% LeanDojo & 57.7 & Temperature Scaling~\citep{temperature} \\ \midrule
% MPTP2078 & 73.0 & NIAGRA~\citep{ensemble}\\ \midrule
% % M2K 98.0, TPTP 82.1
% \end{tabular}}
% \caption{State-of-the-art theorem provers and accuracies on various datasets}
% \label{your-table-label}
% \end{table}




% & NL-PS~\citep{ps_nl_1}& & & &\\
% & NaturalProofs~\citep{naturalproofs}& & & &\\
% & NaturalProofs-Gen~\citep{naturalprover}& & & &\\ 
% & MATcH~\citep{match_2}& & & &\\

% & GamePad~\citep{gamepad}& & & &\\ 
% & CoqGym~\citep{coqgym}& & & &\\ 
% & PRISM~\citep{prism}& & & &\\ 
% & Isabelle 
% & IsarStep~\citep{isarstep}& & & &\\ 
% & PISA~\citep{lisa}& & & &\\ 
% & miniF2F~\citep{minif2f}& & & &\\
% & Magnushammer~\citep{magnushammer}& & & &\\
% & Lean 
% & LeanStep~\citep{pact}& & & &\\ 
% & miniF2F~\citep{minif2f}& & & &\\ 
% & FIMO~\citep{fimo}& & & &\\
% & TRIGO~\citep{trigo}& & & &\\
% & ProofNet~\citep{proofnet}& & & &\\
% & LeanDojo~\citep{leandojo}& & & &\\
% & MLFMF~\citep{mlfmf}& & & &\\
% & HOL Light 
% & HolStep~\citep{holstep}& & & &\\ 
% & HOList~\citep{holist}& & & &\\
% & miniF2F~\citep{minif2f}& & & &\\ 
% & Mizar 
% & MPTP2078~\citep{traditional_ps_2}& & & &\\ 
% & Mizar40~\citep{mizar40}& & & &\\
% & M2K~\citep{rl4tp}& & & &\\
% & Geometry 
% & UniGeo~\citep{unigeo}& & & &\\ 
% & FormalGeo~\citep{formalgeo}& & & &\\
% & Other\\Languages 
% & Holophrasm~\citep{holophrasm}& & & &\\
% & TPTP~\citep{tptp}& & & &\\
% & TacticToe~\citep{tactictoe}& & & &\\
% & MLFMF~\citep{mlfmf}& & & &\\
% & Pre-training\\Corpus 
% & WebMath~\citep{gptf}& & & &\\ 
% & Proof-Pile~\citep{proofnet}& & & &\\ 
% & MathPile~\citep{mathpile}& & & &\\ 
% & OpenWebMath~\citep{openwebmath}& & & &\\
% & Proof-Pile-v2~\citep{llemma}& & & &\\ 
% & DeepSeekMath~\citep{deepseekmath}& & & &\\ 
% & InternLM-Math~\citep{internlm}& & & &\\

% We believe this survey will serve as a foundational resource in deep learning for theorem proving, inspiring and guiding future research in this exciting field.
% , and finally conclude the paper.

% (\S\ref{sec:informal_theorem_proving})
% (\S\ref{sec:formal_theorem_proving})
% (\S\ref{sec:autoformalization})
% (\S\ref{sec:premise_selection})
% (\S\ref{sec:proofstep_generation})
% (\S\ref{sec:proof_search})
% (\S\ref{sec:other_tasks})
% (\S\ref{sec:data_collection})
% (\S\ref{sec:data_generation})
% (\S\ref{sec:metrics})
% (\S\ref{sec:performance})
% (\S\ref{sec:challenges})
% (\S\ref{sec:future_work})


% (\S\ref{sec:conclusion}). 
% In conclusion (\S\ref{sec:conclusion}), we believe this survey will serve as a foundational resource in deep learning for theorem proving, inspiring and guiding future research in this exciting field.




% \paragraph{Contributions.}
% \paragraph{Related work.}
% % compare with existing mathematical reasoning survey / theorem proving survey
% % calculation problem is beyond the scope of this work
% \paragraph{Organizations.}


% 
% Theorem proving is important but needs the expertise and time to write and check the proof. it is obvious for advanced informal math since review time is always long but it applies to the formal theorem proving. For example, four color theorem, Feit–Thompson theorem, compcert, Kepler conjecture,  Gödel's completeness theorem, sel4, mathlib. Despite the non-trivial expertise, existing projects have accumulated a range of data written by human experts, opening up opportunities for machine learning, especially deep learning methods to ease the effort of human experts.

% Using AI to prove theorems dates back to xxx, where xxxxx. From then on, machine learning methods applies to xxxx. With the evolution of deep learning, especially with the deep learning models, recent research xxxx. As shown in Figure xxx, the number of papers in deep learning for theorem proving grew approximately from xxx in 2015 to xxx in 2023. For instance, a line of work try to retrieve helpful lemmas for proving a theorem statement, while some develop LLMs to generate the proof step in ITPs. Despite these advancements, the current state of deep learning for TP presents a complex panorama. Diverse prediction tasks pose a formidable challenge, exacerbated by the varied evaluation metrics, datasets, and settings employed in this area. The lack of a unified framework and clear taxonomy hampers our ability to gauge the true extent of progress achieved and impedes a coherent understanding of the challenges that persist in this evolving field.

%a fragmented landscape of prediction tasks, evaluation metrics, datasets, and methodologies, 

% Despite these advancements, the current state of this field presents a complex panorama. Diverse prediction tasks pose a formidable challenge, exacerbated by the varied evaluation metrics, datasets, and settings employed in this area. The lack of a unified framework and clear taxonomy hampers our ability to gauge the true extent of progress achieved and impedes a coherent understanding of the challenges that persist in this evolving field.

% Informal theorem proving refers to establish the truth of mathematical statements through reasoning that is guided by intuition, natural language explanations. This approach mirrors the natural way individuals learn and apply theorem proving in everyday scenarios. For instance, to prove the Fundamental Theorem of Arithmetic in Figure~\ref{fig:example}~(Top), one must comprehend basic concepts like prime numbers and apply the proven results about primes to conclude. Despite the ubiquity of informal theorem proving, as mathematics evolves, the theories and proofs tend to be more intricate, making verifying their correctness increasingly difficult. 

% This is how mathematical proof is typically taught in the real world, where people prove theorems based on their conceptual understanding of concepts and previously learned knowledge. 
% This approach often relies on the conceptual understanding of the problem at hand, verbal arguments, examples, and sometimes even physical models or analogies to support the reasoning process.


% writing mathematical definitions, theorems, and proofs using natural language and mathematical notations. 


% Jack: We may rewrite the part
% ". This is how mathematics ... and apply the proven results about primes to conclude" 
% to 
% ", which is the most common way to express mathematics. Writing an informal proof for a theorem only requires iteratively applying relevant lemmas to make progress toward or rewrite the conclusion, like the proof of the Fundamental Theorem of Arithmetic in Figure~\ref{fig:example}~(Top)"


%Furthermore, a notable challenge in informal theorem proving is the prevalence of implicit reasoning, where mathematicians might skip steps or overlook minor cases, assuming these to be obvious to the reader. While implicit reasoning may make the proof more concise, it could also lead to gaps or inaccuracies, making errors harder to spot. Famous examples include the Yamabe problem~\citep{yamabe} and Shizuo Kakutani's pesky lemma~\citep{kakutani}.

\section{Lists of Datasets and State-of-the-Art Theorem Provers}
\begin{table}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llllll}
        \toprule[1pt]
        \textbf{Category} & \textbf{Dataset} &\textbf{Language}\tablefootnote{NL stands for natural language. DSL stands for the domain-specific language.} & \textbf{Size}\tablefootnote{We use the number of tokens for pre-training datasets and the number of instances for others.} & \textbf{Source} & \textbf{Target Task}\\
        \midrule
         \multirow{4}{*}{Informal} & NL-PS~\citep{ps_nl_1} & NL &  20,401 & ProofWiki & premise selection \\
         & NaturalProofs~\citep{naturalproofs}& NL & 80,795 & ProofWiki, Stacks, textbooks & PS\\ 
         & NaturalProofs-Gen~\citep{naturalprover}& NL& $\sim$14.5K & NaturalProofs & PG \\ 
        \midrule
        \multirow{14}{*}{Formal} & GamePad~\citep{gamepad} & Coq & 1,602 & Feit-Thompson theorem &\\ 
        & CoqGym~\citep{coqgym}& Coq& 71K& Software Project&\\ 
        & PRISM~\citep{prism}& Coq& - & Software Project&\\ 
        & IsarStep~\citep{isarstep}& Isabelle & 859,759 & AFP&\\ 
        & PISA~\citep{lisa}& Isabelle & $\sim$183K & AFP&\\ 
        
        & Magnushammer~\citep{magnushammer}& Isabelle & $\sim$4.4M & AFP & Premise Selection\\
        & LeanStep~\citep{pact}& Lean & & Mathlib&\\ 
        & TRIGO~\citep{trigo}& Lean & 427 & Trigonometry &\\
        & LeanDojo~\citep{leandojo}& Lean & 98,734 & Mathlib &Premise Selection\\
        & MLFMF~\citep{mlfmf}& Lean, Agda& - &Libraries of Formalized Mathematics &\\
        & HolStep~\citep{holstep}& HOL Light & 2,209,076 & Multivariate Analysis \& Kepler conjecture & Premise Selection\\ 
        & HOList~\citep{holist}&HOL Light  &29,462 & Kepler conjecture &\\
        & MPTP2078~\citep{traditional_ps_2}&Mizar  & 2,078&Mizar Mathematical Library &\\ 
        & Mizar40~\citep{mizar40}&Mizar  & 32,524& Mizar Mathematical Library &\\
        & M2K~\citep{rl4tp}&Mizar  & 2,003& Mizar Mathematical Library&\\

        & Holophrasm~\citep{holophrasm}& Metamath & $\sim$1.923M& Metamath set.mm & Premise Selection\\
        & TPTP~\citep{tptp}& SMT-LIB v2 & 2,752& Miscellaneous &\\
        & TacticToe~\citep{tactictoe}& HOL4 & - & - &\\
        \midrule
        \multirow{5}{*}{Informal \& Formal} 
        & FIMO~\citep{fimo}& Lean & 149 & IMO& Informal+Formal\\
        & ProofNet~\citep{proofnet}& Lean & 371 & Undergraduate-Level Mathematics &Informal+Formal\\
        & miniF2F~\citep{minif2f}& Isabelle & 488 & High-School Competition&\\
        & UniGeo~\citep{unigeo}& DSL & 9,543& High School Curriculum &Diagrams Included\\ 
        & FormalGeo~\citep{formalgeo}& DSL & 133,818 & IMO&\\
        \midrule
        \multirow{7}{*}{Pre-training} & WebMath~\citep{gptf} & NL & 16B & Miscellaneous&\\ 
        & Proof-Pile~\citep{proofnet}& NL & 8.3B & Miscellaneous&\\ 
        & MathPile~\citep{mathpile}& NL &  9.5B & Miscellaneous&\\ 
        & OpenWebMath~\citep{openwebmath}& NL & 14.7B&Miscellaneous &\\
        & Proof-Pile-v2~\citep{llemma}& NL  &55B &Miscellaneous &\\ 
        & DeepSeekMath~\citep{deepseekmath}& NL &120B  & Miscellaneous&\\ 
        & InternLM-Math~\citep{internlm}& NL  &125B & Miscellaneous&\\
        \bottomrule[1pt]
    \end{tabular}
    }
    \caption{Datasets in Theorem Proving}
    \label{tab:app_dataset}
\end{table}


% Original:

% \begin{table}[h]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{llllll}
%         \toprule[1pt]
%         \textbf{Dataset} &\textbf{Language}\tablefootnote{NL stands for natural language. DSL stands for the domain-specific language.} & \textbf{Size}\tablefootnote{We use the number of tokens for pre-training datasets and the number of instances for others.} & \textbf{Source} & \textbf{Target Task}\\
%         \midrule
%         NL-PS~\citep{ps_nl_1} & NL &  20,401 & ProofWiki & premise selection \\
%         NaturalProofs~\citep{naturalproofs}& NL & 80,795 & ProofWiki, Stacks, textbooks & PS\\ 
%         NaturalProofs-Gen~\citep{naturalprover}& NL& $\sim$14.5K & NaturalProofs & PG \\ 
%         \midrule
%         GamePad~\citep{gamepad} & Coq & 1,602 & Feit-Thompson theorem &\\ 
%         CoqGym~\citep{coqgym}& Coq& 71K& Software Project&\\ 
%         PRISM~\citep{prism}& Coq& - & Software Project&\\ 
%         IsarStep~\citep{isarstep}& Isabelle & 859,759 & AFP&\\ 
%         PISA~\citep{lisa}& Isabelle & $\sim$183K & AFP&\\ 
        
%         Magnushammer~\citep{magnushammer}& Isabelle & $\sim$4.4M & AFP & Premise Selection\\
%         LeanStep~\citep{pact}& Lean & & Mathlib&\\ 
%         TRIGO~\citep{trigo}& Lean & 427 & Trigonometry &\\
%         LeanDojo~\citep{leandojo}& Lean & 98,734 & Mathlib &Premise Selection\\
%         MLFMF~\citep{mlfmf}& Lean, Agda& - &Libraries of Formalized Mathematics &\\
%         HolStep~\citep{holstep}& HOL Light & 2,209,076 & Multivariate Analysis \& Kepler conjecture & Premise Selection\\ 
%         HOList~\citep{holist}&HOL Light  &29,462 & Kepler conjecture &\\
%         MPTP2078~\citep{traditional_ps_2}&Mizar  & 2,078&Mizar Mathematical Library &\\ 
%         Mizar40~\citep{mizar40}&Mizar  & 32,524& Mizar Mathematical Library &\\
%         M2K~\citep{rl4tp}&Mizar  & 2,003& Mizar Mathematical Library&\\

%         Holophrasm~\citep{holophrasm}& Metamath & $\sim$1.923M& Metamath set.mm & Premise Selection\\
%         TPTP~\citep{tptp}& SMT-LIB v2 & 2,752& Miscellaneous &\\
%         TacticToe~\citep{tactictoe}& HOL4 & - & - &\\
%         \midrule
%         FIMO~\citep{fimo}& Lean & 149 & IMO& Informal+Formal\\
%         ProofNet~\citep{proofnet}& Lean & 371 & Undergraduate-Level Mathematics &Informal+Formal\\
%         miniF2F~\citep{minif2f}& Isabelle & 488 & High-School Competition&\\
%         UniGeo~\citep{unigeo}& DSL & 9,543& High School Curriculum &Diagrams Included\\ 
%         FormalGeo~\citep{formalgeo}& DSL & 133,818 & IMO&\\
%         \midrule
%         WebMath~\citep{gptf} & NL & 16B & Miscellaneous&\\ 
%         Proof-Pile~\citep{proofnet}& NL & 8.3B & Miscellaneous&\\ 
%         MathPile~\citep{mathpile}& NL &  9.5B & Miscellaneous&\\ 
%         OpenWebMath~\citep{openwebmath}& NL & 14.7B&Miscellaneous &\\
%         Proof-Pile-v2~\citep{llemma}& NL  &55B &Miscellaneous &\\ 
%         DeepSeekMath~\citep{deepseekmath}& NL &120B  & Miscellaneous&\\ 
%         InternLM-Math~\citep{internlm}& NL  &125B & Miscellaneous&\\
%         \bottomrule[1pt]
%     \end{tabular}
%     }
%     \caption{Datasets in Theorem Proving}
%     \label{tab:app_dataset}
% \end{table}


% \begin{table}[h]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule[1pt]
% \textbf{Language} & \textbf{Dataset} &  \textbf{Best Accuracy} & \textbf{Theorem Prover} \\ 
% \midrule
% Coq & CoqGym & 33.8 & Diva~\citep{diva} \\
% \midrule
% \multirow{4}{*}{Lean}& Mathlib (valid/test) & 75.8/77.1 & lean-gym~\citep{curriculum_learning}\\ 
% & LeanDojo & 57.7 & Temperature Scaling~\citep{temperature} \\ 
% % & ProofNet (Proving) & 14.2 & DS-Prover~\citep{dsprover}\\ % Can we remove this?
% & ProofNet & 53.2 & type-check~\citep{typechecking}\\ 
% & miniF2F (valid/test) & 60.2/52.0 & DeepSeek-Prover~\citep{deepseekprover}\\\midrule
% \multirow{2}{*}{Isabelle} & miniF2F (valid/test) & 57.0/51.2 & LEGO-Prover~\citep{lego}/Lyra~\citep{lyra} \\
% & PISA & 71.0 & Magnushammer~\citep{magnushammer} \\\midrule


% Metamath & set.mm (valid/test) & 68.6/58.8 & HTPS~\citep{htps}\\\midrule
% Mizar & MPTP2078 & 73.0 & NIAGRA~\citep{ensemble}\\ 
% \bottomrule[1pt]
% \end{tabular}}
% \caption{Summary of state-of-the-art theorem provers and their best accuracies on several key datasets across different formal languages.}
% \label{tab:app_methods}
% \end{table}




% WebMath~\citep{pact} (35B), Proof-Pile~\citep{proofnet} (8.3B), MathPile~\citep{mathpile} (9.5B), OpenWebMath~\citep{openwebmath} (14.7B), Proof-Pile-2~\citep{llemma} (55B), DeepSeekMath~\citep{deepseekmath} (120B) and InternLM~\citep{internlm} (125B).
% miniF2F~\citep{minif2f} manually translates Olympiad-level problems into 4 formal languages and FIMO~\citep{fimo} formalize the theorem statements of IMO problems in Lean. For undergraduate-level mathematics, ProofNet formalizes problems from textbooks in Lean, and PutnamBench~\citep{putnambench} formalizes the William Lowell Putnam Competition problems in both Lean and Isabelle. 


 % For example, INT generate inequality problems, AlphaGeometry~\citep{alphageometry} generate the meaningful problems with minimal spaning tree. MetaGen also trains a neural generator to synthesize theorems similar to human-written ones.

% performing forward reasoning to sample axiom and arguments with production rules to form a theorem.




% Synthetic datasets rely on algorithmic generation and can form huge mathematical data unrestricted by existing datasets, thus mitigating the issue of data scarcity.

% take any “unsuccessful”
% trajectory in a goal-based task and convert it into a successful one by treating the final state
% as if it were the goal state, in hindsight

% . In these methods, only new proofs are synthesized and the synthetic proofs are only for existing human theorems; no new theorems are synthesized.


% Mustard uses random sampling + LLM+ATP to obtain informal statement+proof+translated formal proof.
% rule-based 
% ~\citet{int} first proposed a rule-based algorithm to generate theorems by iteratively applying axiom to the logic statement in the order and constructed a benchmark INT for inequality problems, leading to the follow-up works ~\citet{polu2020generative,wu2021lime,firoiu2021training,liu2022learning,kazemi2023geomverse}. AlphaGeometry~\citep{trinh2024solving} incorporated the same idea into geometric proof generation for LLM to train on. On the other hand, ~\citep{wang2020learning} trained a machine-learning theorem generator, and ~\citet{palermo2022synthetic,trigo} directly applied off-the-shelf LLMs for theorem and proof generation verified by proof assistant. \\
% expert iteration
% The expert iteration, consisting of iteratively training models on their previously sampled trajectories, was first introduced by ~\citet{silver2017mastering, anthony2017thinking}. Inspired by this, ~\citet{polu2020generative,polu2022formal,mustard} proposed to synthesize proof data by iterative training and fine-tuning a model from its previous output and interacting with ITP, which can generate proofs for harder theorems than the rule-based approaches do. \\
% reinforcement learning
% Reinforcement learning opens another avenue for synthetic data.
% Reinforcement learning opens another avenue for synthetic data.
% \\HOList~\citep{holist}, tf-idf~\citep{bansal2019learning} use randomly sample and learn to prove new theorems in reinforcement learning loop; rlCoP~\citep{kaliszyk2018reinforcement}, HyperTree~\citep{htps} use the exploration-exploitation algorithm in MCTS to explore new theorems; Inspired by the Hindsight Experience Replay in ~\citep{andrychowicz2017hindsight}, ~\citep{aygun2022proving} generates auxiliary theorems with proofs by turning clauses in proof attempts into hindsight for incremental learning. LEGO-Prover~\citep{lego} learns a growing library of theorems by interacting with provers and revolvers.


% MMA + mustard 


%

% IMO, research-level math?

%In terms of evaluation, most works in autoformalization and premise selection apply different metrics and datasets in experiments, complicating evaluating these approaches. In addition, despite the success rate on miniF2F has been widely accepted in evaluating theorem provers, the amount of computational resources and maximum amount of allowed attempts still diverge. 

% For premise selections, LLM-based (e.g. Magnushammer) and DPR-based (e.g. LeanDojo) approaches essentially rely on computing cosine similarity between proof state and premise, which may not select the necessarily logically relevant ones, thus limiting their performances. 



% real-world theorem proving data generation

% structure-aware/hierarchical premise selection/ knowledgebase

% experiments & exploration, e.g., besides proving theorems, mathematicians also perform calculations, inspect numerical data, and finding examples or counter examples


% synergies with formal verification, e.g., synthesizing inductive invariants


% education

% dl for theorem proving application verification/education, breakthroughs in Math and Science

% Conjecturing represents a fundamental aspect of mathematics that extends far beyond the straightforward proving of theorems. It involves mathematicians in identifying the underlying structures of certain problems, formulating conjectures, developing examples or counterexamples, and then proving.
% There is a lot more to mathematics than proving theorems~\citep{towards_math}. Mathematicians identify problem structures, formulate conjectures, and develop examples or counterexamples. 

% For example, core to AlphaGeometry~\citep{alphageometry}'s success is a data generator for synthesizing millions of geometry theorems and proofs. Generalizing this kind of conjecturing capability to other domains may lead to significant improvements in AI for mathematics.



% Existing methods rely extensively on human-written proofs for supervised learning. The amount of proof data is growing but is still far behind other domains where LLMs are successful, e.g., code generation. The largest corpora of formal Isabelle proofs, Archive of Formal Proofs, currently contains 250K proofs. Lean's mathlib contains 140K proofs. This amount of data is decent for small models (e.g., billions of parameters) but insufficient for models with hundreds of billions of parameters. How to fully harness scaling laws is still an open problem in theorem proving. Furthermore, autoformalization is even more data-scarce, due to the difficulty in obtaining aligned informal-formal pairs.



% Generalizability: Mention AlphaGeometry, Lyra, etc.


% Draft: 
% Sufficient high-quality mathematical Datasets underpin the mathematical reasoning capabilities of LLM. Existing informal-to-formal aligned mathematical datasets are scarce in light of the gain from pertaining LLM on large datasets~\citep{gptf}, even the largest source ~\href{https://www.isa-afp.org/}{Isabelle Archive of Proof} has a size of only 322 MB. Also, existing approaches in autoformalization heavily rely on inefficient manual curation or autoinformalization without correctness guarantees, making theorem provers difficult to learn from abundant informal mathematical resources, thus a bottleneck in theorem proving.



% Draft: Existing challenges in deep learning for theorem proving are manifested in disunified metrics for experiments, lack of aligned data for training, and difficulty in generalizing to new domains.

% This section summarizes key metrics and benchmark approaches in autoformalization, premise selection, and theorem proving.

% Existing evaluation metrics for autoformalization involve manual inspection and automated metrics, including the compilation rate to check whether a formalization is syntactically correct, and the BLEU score to compute semantic similarity. 
% , with secondary consideration given to automated metrics such as the compilation rate and BLEU score.






% \subsection{Metrics}
% \label{sec:metrics}
% Existing evaluations for autoformalization involve manual inspection and automated metrics to balance accuracy and scalability. Manual equivalence checking is accurate but requires significant expertise and labor. In contrast, automated metrics such as the compilation rate assess only syntactic correctness without comparing with the ground truth, and the BLEU score is susceptible to misclassifying formalizations semantically similar but not logically equivalent to the ground truth ones, leading to false positives.
% % Evaluating autoformalization involves balancing precision and scalability. Manual equivalence checking, while accurate, requires significant expertise and labor, limiting its scalability. In contrast, automated metrics like the compilation rate and BLEU score~\citep{bleu} offer scalability but may not fully capture logical accuracy: the compilation rate may include semantically wrong but syntactically correct formalizations, and the BLEU score may overlook semantically correct formalizations that differ from human-written ones.
% Classification metrics are widely used for evaluating premise selection. For example, recall at $k$ ($R@k$) measures the ratio of correctly used premises in ground-truth proof within the top-k selections, and the mean reciprocal rank (MRR) computes the average reciprocal rank of the first useful selected premise. However, these metrics might neglect other valid premises for alternative correct proofs different from the ground-truth ones, causing false negatives. 
% % In premise selection, metrics such as Recall at $k$ ($R@k$) and Mean Reciprocal Rank (MRR) are often used to assess the selected $k$ premises based on their presence in ground-truth proofs. However, these metrics might neglect other valid premises for alternative correct proofs different from the ground-truth ones. Integrating premise selection with proof generation in evaluations provides another measure of its impact, though accurately assessing the performance of premise selection alone remains challenging.
% % The overall theorem-proving approaches can be evaluated by the success rate of theorems proved in a dataset. 
% For proofstep generation and proof search, current approaches mainly merge these processes to evaluate the overall performance through the success rate of theorems proved in a test set. 
% % However, this metric is still complicated by various experimental setups: some studies impose a time budget, while others restrict the number of proof searches or LLM queries.

% \subsection{Performance}
% \label{sec:performance}
% Using manual checking, \citet{autoformalization_llm} and \cite{proofnet} show that state-of-the-art LLMs with few-shot prompting can correctly formalize 25\% and 13\% statements from high-school and undergraduate-level problems, which demonstrates the challenge inherent in autoformalization. Nevertheless, both studies reveal that LLMs exhibit considerably higher efficacy in informalization, achieving around 76\% and 62\% accuracy. 
% % Despite the modest success in autoformalizing statements, 
% Subsequent research~\citep{dsp, denigma, lego} reveals the value of formalizing the informal intermediate goals to prove theorems in modularized pipelines.

% Fine-tuned BERT-based retrieval models have significantly improved over traditional methods, demonstrating a remarkable ability to generalize to unseen data for premise selection. For example, ReProver~\citep{leandojo} achieves 27.6\% for R@10 and 0.24 for MRR on the LeanDojo benchmark for retrieving unseen premises in training, while BM25~\citep{bm25} achieves 15.5\% for R@10 and 0.14 for MRR. Furthermore, when combined with a tactic prediction model Thor~\citep{thor}, Magnushammer~\citep{magnushammer} improves the traditional premise selection methods in Sledgehammer~\citep{sledgehammer} with a success rate from 57\% to 71\% on the PISA dataset and from 28.3\% to 36.9\% on the miniF2F-valid dataset, respectively.

% For proof generation, recent researches~\citep{dsp, denigma, lyra, lego} demonstrate remarkable performance increases using state-of-the-art LLMs like GPT-4 in structured frameworks than tactic-based models with best-first search heuristic. For instance, LEGO-Prover~\citep{lego} achieve 57.0\% accuracy and 50.0\% accuracy on the valid and test set of miniF2F, while previous best tactic models Thor~\citep{thor} with expert iteration training~\citep{autoformalization_llm} achieve 37.3\% and 35.2\%. Moreover, using deep learning guided proof search could further improve the performance of both ITPs and ATPs. HTPS~\citep{htps} achieve an accumulative successful rate of 58.6\% on miniF2F-valid through online training and a 41.0\% pass rate with 64 search attempts on miniF2F-test. Besides, the reinforcement learning-based ATP prover NIAGRA~\citep{ensemble} outperforms both the sophisticated E and Vampire on the MPTP2078 dataset.

% to 71\% in PISA, 

% and from 28.3\% and 29.9\% to 36.9\% and 37.3\% on miniF2F validation and testing dataset. .



% The miniF2F test set emerges as a comprehensive benchmark for theorem prover evaluation. The LLM-based LEGO-Prover, leveraging GPT-4 and an expanding skills library, achieved a leading 50.0\% success rate (pass @ 100), surpassing the HTPS prover ~\citep{htps}, which integrates MCTS search and online training, with a 41.0\% pass @ 64. This indicates the dominance of LLMs over search algorithms in theorem proving, highlighting the potential of combining these methodologies. On the Lean Mathlib dataset, the expert iteration-based lean-gym prover records the highest pass rate @ 64 of 77.1\%. Nonetheless, Coq datasets like CoqGym remain a significant challenge, with the best Coq prover, passport ~\citep{passport}, achieving only a 17.2\% success rate.

% Furthermore, integrating premise selection model with  has markedly boosted theorem provers, as evidenced by Thor\citep{thor} and Magnushammer\citep{magnushammer}, which elevated the performance of the Sledgehammer tool from 38.3\% to a leading 71.0\% success rate on PISA.

% Rapid advancements in premise selection have also been reported. The DPR-based retriever \citep{leandojo} doubled the performance of the traditional BM25 retriever to a Recall @ 10 of 38.4\% in the LeanDojo benchmark. Similarly, a contrastively-finetuned natural premise retriever \citep{ps_contrastive} achieved 36.9\% on NaturalProofs, significantly outperforming the BERT model's 20.3\%. Integrating premise selection approaches has markedly boosted theorem provers, as evidenced by Thor\citep{thor} and Magnushammer\citep{magnushammer}, which elevated the performance of the Sledgehammer tool from 38.3\% to a leading 71.0\% success rate on PISA.

% Despite the low accuracy for autoformalizing statements, DSP~\citep{dsp} and LEGO~\citep{lego} demonstrate the usefulness of autoformalizing the informal proofs when proving a theorem, improving previous state-of-the-art methods from 35\% to 39\% and 50\%.

% using informal proofs with autoformalization could significantly improve the performance of


% Leading autoformalization tools, as identified by ~\citet{proofnet, autoformalization_llm}, have shown accuracies of 16.1\% and 25.3\% on ProofNet and a select 150-theorem subset of MATH, respectively, underscoring the challenges in autoformalizing advanced mathematical content. Nevertheless, studies by ~\citet{autoformalization_llm} and ~\citet{mma} reveal that Large Language Models (LLMs) exhibit superior performance in autoinformalization compared to autoformalization. Furthermore, autoformalization tools significantly improve theorem provers, for instance, the DSP approach~\citep{dsp} increase Sledgehammer's proof success rate on the miniF2F-test from 10.4\% to 37.7\%.





% \begin{table}
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
% Dataset & SOTA accuracy (valid/test) & Prover\\ \hline
% mathlib & 75.8/77.1 & lean-gym~\citep{curriculum_learning}\\ \hline
% minif2f & 57.0/50.0 & LEGO-Prover~\citep{lego} \\ \hline
% proofnet & 14.2 & DS-Prover~\citep{dsprover}\\ \hline
% pisa & 71.0 & Magnushammer~\citep{magnushammer} \\ \hline
% metamath & 68.6/58.8 & HyperTree~\citep{htps} \\ \hline
% HOList & 49.95 & GNN~\citep{graph_representation} \\ \hline
% LeanDojo & 57.7 & Temperature Scaling~\citep{temperature} \\ \hline
% MPTP2078 & 73.0 & NIAGRA~\citep{fokoue2023ensemble}\\ \hline

% \end{tabular}
% \caption{State-of-the-art theorem provers and accuracies on various datasets}
% \label{your-table-label}
% \end{table}

% Autoformalization:
% \\ProofNet: Code-DaVinci-002 with Prompt Retrieval 16.1
% \\Premise Selection:
% \\LeanDojo: GPT4 with R @ 10: 38.4\%
% \\NaturalProofs: ctpt-webmath~\citep{ps_contrastive} with R @ 10: 36.9\%
% \\Theorem Proving

% To be summarized: NIAGRA~\citep{fokoue2023ensemble} set significant benchmarks for ATP with a success rate of 75.5\% in Mizar MPTP2078 and 84.6\% with Vampire on TPTP. In the Isabelle environment, LEGO-Prover~\citep{lego} achieved state-of-the-art results on miniF2F with accuracies of 57.0\% and 50.0\%, whereas . In Lean, DS-Prover~\citep{dsprover} together with an Optimized LeanDojo~\citep{leandojo} attained a 14.2\% success rate on ProofNet~\citep{proofnet}, while lean-gym~\citep{curriculum_learning} achieved non-sota results of 47.3\%/36.6\% on miniF2F but sota outcomes of 75.8\%/77.1\% on mathlib. Lastly, the Passport~\citep{passport} is the best Coq-based theorem prover, attained 17.2\% on CoqGym dataset. 

% (Informalization)

% We evaluate the theorem-proving techniques on mathematical datasets over autoformalization, premise selection, and theorem-proving in the past two years. In autoformalization task, the Codex model with premise retrieval~\citep{proofnet} achieves a compilation rate and translation accuracy of 45.2\% and 16.1\% on ProofNet. 
% In premise selection, the baseline GPT-4 model achieves 38.4\% Recall @ 10 on LeanDojo, and the ctpt-webmath~\citep{ps_contrastive} achieves 36.9\% on NaturalProofs~\citep{naturalproofs}. In the realm of premise selection, GPT4's baseline on the LeanDojo Benchmark~\citep{leandojo} achieved Recall @ 10 of 38.4\%, while in the informal premise selection, the contrastively fine-tuned model on WebMath~\citep{ps_contrastive} achieved Recall @ 10 of 36.92\% on NaturalProofs~\citep{naturalproofs}, which is a huge improvement comparing with 23.76\% for BERT.
% In theorem proving, NIAGRA~\citep{fokoue2023ensemble} set significant benchmarks for ATP with a success rate of 75.5\% in Mizar MPTP2078 and 84.6\% with Vampire on TPTP. In the Isabelle environment, LEGO-Prover~\citep{lego} achieved state-of-the-art results on miniF2F with accuracies of 57.0\% and 50.0\%, whereas Magnushammer~\citep{magnushammer} combined with Thor~\citep{thor} reached a 71.0\% proof rate on PISA~\citep{lisa}. In Lean, DS-Prover~\citep{dsprover} together with an Optimized LeanDojo~\citep{leandojo} attained a 14.2\% success rate on ProofNet~\citep{proofnet}, while lean-gym~\citep{curriculum_learning} achieved non-sota results of 47.3\%/36.6\% on miniF2F but sota outcomes of 75.8\%/77.1\% on mathlib. Lastly, the Passport~\citep{passport} is the best Coq-based theorem prover, attained 17.2\% on CoqGym dataset. 




% Autoformalization
% ProofNet and miniF2F are pivotal datasets for evaluating autoformalization capabilities. The Code-DaVinci-002 baseline demonstrates an accuracy of 13.4\% and a compilation rate of 23.7\% on ProofNet~\citep{proofnet}, and 25.3\% accuracy on a MATH dataset subset~\citep{agrawal2022towards}. Fine-tuning the LLaMA-33B model on MMA~\citep{mma} further improved compilation rates to 36\% on miniF2F and 30\% on ProofNet. GPT3-turbo, applied to 50 theorems from arXiv2Formal, achieved a 17.2 BLEU score and a 140.5 TER score~\citep{autoformalization_new_approach}. In the realm of GSM8K, DTV~\citep{dtv} notably enhanced Minerva 62B's accuracy from 48.6\% to 71.4\%, which increased to 79.4\% when used with GPT3. DSP~\citep{dsp} significantly improved Minerva 62B's performance on the miniF2F dataset, from 28.3\%/29.9\% to 43.9\%/37.7\% on valid/test splits.
% % Premise Selection
% For premise selection, most studies utilize Recall @ 10 (R@10) or Precision @ 10 (P@10) metrics. Within this context, GPT4's baseline on the LeanDojo Benchmark~\citep{leandojo} achieved a 38.4\% R@10. NaturalProofs~\citep{naturalproofs} saw R @ 10 scores of 23.76\% for BERT and 36.92\% for ctpt-webmath. ColBERT~\citep{zhong2022evaluating} achieved a P@10 of 21.3\% on ARQMath-2.
% % state-of-the-art performance on several datasets (i.e., public, widely used)
% In traditional Automated Theorem Proving (ATP), NIAGRA~\citep{fokoue2023ensemble} set significant benchmarks with performances of 75.5\% in an unsupervised learning setup on Mizar MPTP, 99.0\% with Vampire on M2K~\citep{kaliszyk2018reinforcement}, and 84.6\% with Vampire on TPTP, outshining other ATP systems. In the Isabelle environment, LEGO-Prover~\citep{lego} achieved state-of-the-art results on miniF2F with accuracies of 57.0\% and 50.0\%, whereas Magnushammer~\citep{magnushammer} combined with Thor~\citep{thor} reached a 71.0\% proof rate on PISA~\citep{lisa}. In Lean, DS-Prover~\citep{dsprover} together with an Optimized LeanDojo~\citep{leandojo} attained a 14.2\% success rate on ProofNet~\citep{proofnet}, while lean-gym~\citep{curriculum_learning} achieved non-sota results of 47.3\%/36.6\% on miniF2F but sota outcomes of 75.8\%/77.1\% on mathlib.




% GPT3.5-Turbo arXiv2Formal~\citep{autoformalization_new_approach} 41.7 83.9 33.1 (BLEU/TER/TrueSkill
% )
% DTV~\citep{dtv}: Improvement of Autoformalization. DTV Formalization with GPT3.5 on GSM8K: 79.4\%

% DSP: Same as above. 
% MMA (LLaMA 33B) Compilation rates (\%): 36\% on Isabelle miniF2F and 30\% on Isabelle 
% Lean4 formalisations are acceptable with minor corrections.

% ProofNet: Codex (prompt retrieval) 45.2 14.8 16.1 (Typecheck rate/BLEU/Accuracy)

% Codex (~\citep{autoformalization_llm}) Isabelle: 38 perfect translation (25\%) on 150 randomly selected MATH

% BLEU Score: 57.13 43.33 (miniF2F 130 algebra, miniF2F 110 number\_theory)

% Premise Selection
% 298 randomly selected theorems from MPTP2078 in TPTP format~\citep{sennrich-etal-2016-improving}: Transformer has 0.56 Coverage score.



% proves theorems in a level-by-level manner, recursively generating a verifiable sketch of the proof at each level and solving the current level’s theorem or conjecture using GPT-4.

% searches for different levels of verifiable proof sketches and proves the given theorem in a recursive, level-by-level manner.

% Alternative works~\citep{dsp, denigma, lyra, copra, lego,} leverage autoformalization to generate the formal proof of an informal problem in structured pipelines. 

% These approaches decompos the informal proofs into sub-goals and leveraging autoformalization and other  to prove these sub-goals. For instance, Lyra~\citep{lyra} leverages two correction mechanisms to refine the wrong proofs from GPT-4. 
% LEGO-Prover~\citep{lego} decomposes the informal proofs to sub-goal lemmas, proves or retrieves lemmas from a growing library, and finalizes the theorem using these lemmas.

% of a dynamic proof of polynomial inequalities.

% AutoTrig~\citep{trigo_rl} applies imitation learning and proximal policy optimization~\citep{ppo} to train its policy and value networks to prove trigonometric identities.%  peano, drl4hol, without_imitation,  longer_proofs0, 



% including type inference, suggesting missing assumptions and completing equalities using self-supervised language modeling.   further proposes nine self-supervised auxiliary tasks by masking various sub-terms in human proofs. Recently, 


% In addition to core theorem proving tasks, various studies have introduced complementary prediction tasks enhancing theorem proving capabilities. \citet{gamepad, ps_gnn_1, curriculum_learning} focus on predicting the remaining proof length for a given goal. Skip-tree~\citep{skip-tree} introduces tasks for type inference, assumption suggestion, and equality completion through self-supervised language modeling. IsarStep~\citep{isarstep} aims at predicting intermediate propositions within proofs. LIME~\citep{lime} develops tasks targeting deduction, abduction, and induction to support pretraining. PACT~\citep{pact} innovates with nine self-supervised auxiliary tasks, involving the masking of sub-terms in proofs. Additionally, recent work by \citet{match_1, match_2} focuses on matching proofs with statements from extensive databases.


% Beyond the primary tasks previously outlined, our survey briefly examines additional predictive tasks that support or intersect with theorem proving. Works such as \citet{gamepad, ps_gnn_1, curriculum_learning} focus on estimating the remaining length of a proof. Skip-tree~\citep{skip-tree} introduces tasks like type inference, assumption suggestion, and equality completion via self-supervised language models. IsarStep~\citep{isarstep} aims at predicting intermediate propositions based on surrounding proofs. LIME~\citep{lime} designs tasks for deduction, abduction, and induction as a pretraining strategy. PACT~\citep{pact} innovates with nine self-supervised auxiliary tasks, involving the masking of sub-terms in existing human proofs. Recently, research by \citet{match_1, match_2} has moved towards matching proofs with statements from extensive databases.

% \citet{lazycop, lazycop2} uses GNN with A* search in tableux prover.
% \citet{components} trains gnn with previous clause information to guide E
% \citet{fast_slow} combines gnn and gbdt to guide e

% holophrsam~\citep{holophrasm, metagen} uses GRU to guide Monte Carlo Tree Search (MCTS) for MetaMath. 
% TacticToe uses nn to predict the cost function in A* search. \citet{proof_search_propositional} guides the search in automated proof synthesis in the order of the likelihood

% \citet{ps_gnn_2} uses GNN to guide MCTS for leanCoP.
% \citet{neural_guided_tp} use gnn to guide lerna

% \citep{synthetic_theorems} uses GNN/MLP for saturation-based solver

% INT~\citep{int} trains gnn to estimate the value of a state + mcts
% \citet{plcop} uses gnn + mcts for leancop
% \citet{likelihood_search} tnn + mcts to predict the provability of the goals


% gptf~\citep{gptf} trains a value function using outcome objective in metamath + best. the highest cumulative log probability
% \citet{curriculum_learning} predicts the proofsize objective
% \citet{pact} proposes the best first search. 

% \citet{synthetic_2, her} uses Transformer encoding network as clause scoring network using incremental learning, tptp.


% \citet{lemmas} focus on condensed detachment (CD) problems






% \citet{drl_propositional} uses GNN to predict as the value function in deep reinforcement learning.,
% TRAIL~\citep{trail, experimental_study, trail2, elements, ensemble} use drl on saturation-based prover using enigma features/gnn + attention policy network, policy gradient methods
% ~\citet{without_imitation} uses gnn + rl
% \citet{drl4hol} use drl + mcts using tnn for encoding in hol4.
% \citet{learning_polynomial} uses dqn for polynomial inequalities.
% \citet{longer_proofs0, longer_proofs} uses ppo with statistical features xxcop.
% \citet{smartcoq} uses dqn for coq
% \citet{rl_hol4} uses LSTM to encode + REINFORCE algorithm for hol4
% \citet{3sil, 3sil_2} uses drl on the arithmetic rewriting tasks and combines with prover9
% \citet{tacticzero} uses policy gradient based drl for hol4

% htps~\citep{htps} uses alphazero-like mcts
% \citet{peano} uses reinforcement to learn to policy
% \citet{trigo_rl} uses ppo


% \citep{gym-saturation_1, gym-saturation_2} use rl in iprover and vampire
% \citep{rl4e} uses rl for E
% \citet{geo_drl} use drl + mcts for geometry

% For tactic prediction model in ITPs, main stream of research leverages beam search with DFS~\citep{coqgym, tactok}, BFS~\citep{holist, graph_representation, trigo}, or best-first heuristics~\citep{gptf, pact, curriculum_learning}. Specfically, GPT-$f$~\citep{gptf} trains a value function using outcome objective in language modeling and choose the nodes based on accumulated log probability. \citet{curriculum_learning} further proposes to predict the proofsize objective to guide the search. Recently, COPRA~\citep{copra} leverages gpt4 TO PEROFRM history dependent backtracking search. \citet{llm_mcts} use MCTS to guide llm generate the lean/coq proof






% pertaining tasks for theorem proving, LIME, 
% PACT~\citep{pact} further proposes several self-supervised auxiliary tasks for jointly training a language model alongside the tactic prediction objective.
% proof mathching
% holstep, ISARSTEP, gamepad, ，Mathematical Reasoning in Latent Space，Mathematical Reasoning via Self-supervised Skip-tree Training，Tree Neural Networks in HOL4



% conjecuring~\citep{tableau_rnn, conjecturing_1, conjecturing_2, skip-tree, conjecturing_3}
% analysis

% Tons of Inductive Programs~\citep{tip} 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

